Talk2Data: A Natural Language Interface for Exploratory Visual Analysis via Question Decomposition

Through a natural language interface (NLI) for exploratory visual analysis, users can directly "ask" analytical questions about the given tabular data. This process greatly improves user experience and lowers the technical barriers of data analysis. Existing techniques focus on generating a visualization from a concrete question. However, complex questions, requiring multiple data queries and visualizations to answer, are frequently asked in data exploration and analysis, which cannot be easily solved with the existing techniques. To address this issue, in this paper, we introduce Talk2Data, a natural language interface for exploratory visual analysis that supports answering complex questions. It leverages an advanced deep-learning model to resolve complex questions into a series of simple questions that could gradually elaborate on the users' requirements. To present answers, we design a set of annotated and captioned visualizations to represent the answers in a form that supports interpretation and narration. We conducted an ablation study and a controlled user study to evaluate Talk2Data's effectiveness and usefulness.

==> tables/annotation.tex <==
\begin{table}[!h]
% \vspace{-0.6em}
% \scriptsize
\fontsize{9}{9}\selectfont
\begin{tabular}{p{2cm}p{2cm}p{3.3cm}}
\toprule
% \rowcolor[HTML]{EFEFEF} 
\textbf{Fact} & \textbf{Chart} & \textbf{Annotation} \\ \midrule
Association & Scatter & Lines \\ 
Categorization & Bar & Colors \\ 
Difference & Bar & Text, Lines \\ 
Distribution & Bar, Area & Shapes \\ 
Extreme & Bar, Line & Text, Pointers, Colors  \\ 
Outlier & Line, Area & Text, Pointers, Colors \\ 
Proportion & Pie, Bar & Text, Colors \\ 
Rank & Bar & Text, Colors \\ 
Trend & Line, Bar, Area & Lines \\ 
Value & Bar & Text  \\ 
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{Annotated Charts for Tabular Data}
\label{tab:annotation}
% \vspace{-0.6em}
\end{table}

==> tables/corpus2.tex <==
\begin{table*}[htbp]
    \small
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \def\arraystretch{1.2}
\begin{tabular*}{\linewidth}{lllll}
\hline
\textbf{Question Type} & \textbf{Operator Type} & \textbf{Complex Question}                                                                                                         & \textbf{Decomposed Question}                                                                                                                                    & \textbf{Count} \\ \hline
                       & Cut-Type               & \begin{tabular}[c]{@{}l@{}}Show me some information about book price in the \\ different genre.\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}(1) What are the differences in price between each genre?\\ (2) Which genre has the highest price?\end{tabular}                      & 20.6\%         \\ \cline{2-5} 
Top-Down               & Cut-Measure            & \begin{tabular}[c]{@{}l@{}}Which genre of book is an outlier compare with other \\ books?\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}(1) Which genre of the book has an anomaly user rating.?\\ (2) Which genre of book has an anomaly reviews?\end{tabular}              & 5.82\%         \\ \cline{2-5} 
                       & Cut-Breakdown          & What is the trend of user rating?                                                                                                 & \begin{tabular}[c]{@{}l@{}}(1) What is the trend of user rating over different years?\\ (2) What is the trend of user rating over different years?\end{tabular} & 8.1\%          \\ \hline
                       & Find-Interaction       & Which book is expensive and well-regarded?                                                                                        & \begin{tabular}[c]{@{}l@{}}(1) Which book has a review higher than average?\\ (2) Which book has a price higher than average?\end{tabular}                      & 10.3\%         \\ \cline{2-5} 
Bottom-Up              & Find-Comparison        & \begin{tabular}[c]{@{}l@{}}Which genre has more user reviews, fiction book\\  or non-fiction book?\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}(1) How many reviews the fiction book has? \\ (2) How many reviews the non-fiction book has?\end{tabular}                            & 22.8\%         \\ \cline{2-5} 
                       & Find-Bridging          & \begin{tabular}[c]{@{}l@{}}In the year with most reviews, what is the distribution \\ of price over different genre?\end{tabular} & \begin{tabular}[c]{@{}l@{}}(1) Which year has the highest/lowest reviews?\\ (2 )What is the overall distribution of price over genre ?\end{tabular}             & 28.4\%         \\ \hline
\end{tabular*}
\label{tab:templates}
\caption{Question Template.}
\end{table*}
